Re-Identification Supervised Texture Generation

The estimation of 3D human body pose and shape from a single image has been extensively studied in recent years. However, the texture generation problem has not been fully discussed. In this paper, we propose an end-to-end learning strategy to generate textures of human bodies under the supervision of person re-identification. We render the synthetic images with textures extracted from the inputs and maximize the similarity between the rendered and input images by using the re-identification network as the perceptual metrics. Experiment results on pedestrian images show that our model can generate the texture from a single image and demonstrate that our textures are of higher quality than those generated by other available methods. Furthermore, we extend the application scope to other categories and explore the possible utilization of our generated textures.

==> AblationStudy.tex <==
\subsection{Ablation Study}\label{ablation}
In order to demonstrate the indispensable role that re-identification loss plays in our method, we designed experiments to compare the images generated from different model settings both qualitatively and quantitatively. The qualitative result is shown in Fig.~\ref{ablation_img} while the quantitative result is shown in Table.~\ref{ablation_table}.

\begin{figure*}[h]
	\centering
	\includegraphics[width=0.97\linewidth]{ablation.pdf}
	\caption{\textbf{Qualitative Results.} The result from eight images, of different model settings, is shown with two columns. Each column shows (in order from left): input images (from test set), RGB $\ell_1$ loss, Imagenet-based perceptual loss, Softmax loss, triplet hard loss, re-identification loss using deep features, model without the pose alignment, re-identification loss without PCB module, the re-identification loss proposed in Sec.~\ref{reid-loss}}
	\label{ablation_img}
\end{figure*}

\begin{table*}
	\begin{center}
		\begin{tabular}{l c c c c c c c c}
			\hline
			Model & RGB & Imagenet & Softmax& Triplet&  Deep Feature&No-Pose&No-PCB&ReID Loss\\
			\hline
			SSIM & 0.162 & 0.149& 0.145& 0.148& 0.156& 0.158& 0.159& \textbf{0.164}\\
			mask-SSIM & \textbf{0.374} & 0.356& 0.350& 0.354& 0.363& 0.365& 0.369& 0.372\\
			IS & 3.96 & 4.04& 3.75& 3.87& 3.83& \textbf{4.07}& 3.75& 3.96 \\
			mask-IS & \textbf{2.90} & 2.59& 2.53& 2.43& 2.42& 2.63 & 2.77& 2.52\\
			\hline
		\end{tabular}
	\end{center}
	\caption{\textbf{Quantitative Ablation Study Results.} The inception score is lower than usual, as it is not fit for the image quality evaluation of images from single category.}
	\label{ablation_table}
	
\end{table*}

%In this work, we experimented on the following model settings: \begin{enumerate*}
%	\item Change the loss module to imagenet pre-trained perceptual loss or $\ell_1$ loss of rendered image.
%	\item Use random gathered poses rather than pose estimated by HMR.
%	\item Substitute the re-identification module in loss function to one without PCB.
%	\item Try losses of different re-identification network features.
%\end{enumerate*}
%
%\paragraph{Ablation of network model in re-identification loss.}
%
%In this experiment, we substitute the re-identification loss with the following loss functions:
%RGB loss and perceptual loss.
%
%The result is shown in the columns labeled ``RGB'' and ``Imagenet'' in Fig.~\ref{ablation_img}. The RGB loss is defined as the $\ell_1$ loss between the rendered textured image with the input.
%\begin{equation}
%\mathcal{L}_{RGB}(\mathbf{x},\mathbf{y})=\Vert \mathbf{x} - \mathbf{y} \Vert_1
%\end{equation}
% 
% 
%The model trained with RGB $\ell_1$ loss performs bad in generating details, such as hands and shins, of the image. This is caused by the inaccurate estimation of human body poses and shapes provided by HMR \cite{end2end} module. 
%
%The model trained with Imagenet-based perceptual loss ended up with an even worse result. Though arms and legs generated from the model can be identified, the generation quality of torso is poor. This is because the feature extraction network trained on Imagenet tends to extract the general features of objects rather than concentrating on human body textures. 
%
%The SSIM and mask-SSIM score of RGB loss are among the highest scores in all of the experimental results, this is because the RGB loss optimize the generated texture in a pixel-to-pixel way, which is equivalent to directly optimizing the SSIM score in the training process. In accordance with the perceived quality, the SSIM and mask-SSIM score of perceptual loss is one of the lowest among all results.

\paragraph{Ablation of different loss settings.}

In this experiment, we explored whether different loss settings will influence the performance of generative model. We carried out the experiments with following loss settings and compared them with our proposed re-identification loss: \begin{enumerate*}
	\item Softmax loss.
	\item Triplet hard loss.
	\item $\ell_1$ loss of deep features.
\end{enumerate*}

These loss functions are all based on the re-identification network with PCB. In this network, the image is passed into resnet-50 network and a feature $g_{1}$ of $6 \times 1024$ dimensions is extracted. A full-connected layer is appended and the output feature $g_{2}$ is set to $6 \times 256$ dimensions. This feature is subsequently sent into a full-connected network, which produces the Softmax feature $g_{s}$. 

The Softmax loss in our experiment is defined as the cross-entropy loss between the $g_{s}$ of the generated and input image. The sample images from model trained with Softmax loss is shown in the column labeled ``Softmax'' of Fig.~\ref{ablation_img}. As the Softmax loss is calculated from the features produced by several full-connected layers, a large amount of information for reconstructing human textures is discarded while only the feature for classification is preserved. Thus, the Softmax loss is not a good criteria of texture quality, which makes both the qualitative and quantitative result unsatisfying.

The result of triplet loss is show in the column labeled ``Triplet'' of Fig.~\ref{ablation_img}, which is also far from satisfaction. To explain this, we should trace back to the definition of the triplet loss.
\begin{equation}
\mathcal{L}_{triplet}=[\Vert g_{2}^{\mathbf{y}} - g_{2}^p \Vert_2^2 - \Vert g_{2}^{\mathbf{y}} - g_{2}^n \Vert_2^2 + \alpha]_+ 
\end{equation}

In the definition above, $g_{2}^{\mathbf{y}}$ is the feature of rendered texture image, while $g_{2}^p$ and $g_{2}^n$ is the feature of positive and negative samples respectively. The triplet loss does not optimize the distance between $g_{2}^{\mathbf{y}}$ and $g_{2}^p$ to zero and allows a certain distance between them according to the margin parameter $\alpha$. Moreover, the triplet loss rewards the enlargement of distance between $g_2^{\mathbf{y}}$ and $g_{2}^n$. This might allow $g_{2}^{\mathbf{y}}$ far apart from $g_{2}^p$, which will damage the similarity between rendered image $\mathbf{y}$ and the input image $\mathbf{x}$ in the training process. All of these will have a negative effect on the texture generation task, which is also demonstrated by the SSIM and mask-SSIM scores.

The deep feature loss is defined as the $\ell_1$ distance between deep features of re-identification network. Specifically, it is defined below:

\begin{equation}
\mathcal{L}_{deep} = \Vert (g_{1}^{\mathbf{y}} + g_{2}^{\mathbf{y}}) - (g_{1}^{\mathbf{x}} + g_{2}^{\mathbf{x}}) \Vert_1
\end{equation}

The result of deep $\ell_1$ feature loss is shown in the column labeled ``Deep Feature'' of Fig.~\ref{ablation_img}. Comparing with the re-identification loss in Sec.~\ref{reid-loss}, this result is good while ignoring some details, e.g. the patterns on clothes. This is because the amount of information the deep feature holds is between the Softmax feature and feature for perceptual loss. The result is also indicated by the SSIM and mask-SSIM scores.

\paragraph{With vs. without body pose alignment.}

In our experiments, we estimate the body pose and shape parameters of the images with HMR and render the SMPL body model with these parameters. This can be viewed as the alignment of posture and body position. However, given the re-identification's ability of filtering out the influence of body posture and position, it is meaningful to study the effect of pose alignment on the generative model.

In this experiment, we substitute the SMPL parameters with the randomly chosen parameter from the walking sequences of the CMU MoCap database \cite{cmumocap}. The result is shown in the column labeled ``No pose'' of Fig.~\ref{ablation_img}. The result shows that the model without pose alignment can generate textures of acceptable quality. However, the defects in arm parts indicates the significance of body alignment. Moreover, in the top right example where human only occupies part of the image, the model without pose alignment cannot recovery the human body size and location automatically and it regards the background as a part of the body.

The SSIM and mask-SSIM scores of model without pose alignment are 0.158 and 0.365 respectively. This result indicates that the feature extracted by re-identification model is influenced by the position and posture of the human body. The conclusion made by \cite{alignedreid} is also consistent with our analysis.

\paragraph{With vs. without body part features.}

In our method, we employ PCB model \cite{pcb} as the feature extraction module of re-identification loss because it can extract features from every part of the human body, which is supposed to be beneficial for the reconstruction of body details. To demonstrate this, we compared the generating result of re-identification loss with or without PCB module. In order to exclude the influence caused by the performance of re-identification model, the top-1 accuracy of the two models are both around 92\% on Market-1501 dataset.

The result is shown in the column labeled ``No-PCB'' of Fig.~\ref{ablation_img}. The result with and without body part features is mostly similar while they only differs on the arms or clothing details. This aligns well with the SSIM and mask-SSIM results, where the scores of No-PCB is slightly lower than proposed method. The high quality textures generated by the model without PCB can be ascribed to the high accuracy of re-identification model which extracts precise features.


